Deploying Deep Reinforcement Learning Systems: A Taxonomy of Challenges

Deep reinforcement learning (DRL), leveraging Deep Learning (DL) in reinforcement learning, has shown significant potential in achieving human-level autonomy in a wide range of domains, including robotics, computer vision, and computer games. This potential justifies the enthusiasm and growing interest in DRL in both academia and industry. However, the community currently focuses mostly on the development phase of DRL systems, with little attention devoted to DRL deployment. In this paper, we propose an empirical study on Stack Overflow (SO), the most popular Q&A forum for developers, to uncover and understand the challenges practitioners faced when deploying DRL systems. Specifically, we categorized relevant SO posts by deployment platforms: server/cloud, mobile/embedded system, browser, and game engine. After filtering and manual analysis, we examined 357 SO posts about DRL deployment, investigated the current state, and identified the challenges related to deploying DRL systems. Then, we investigate the prevalence and difficulty of these challenges. Results show that the general interest in DRL deployment is growing, confirming the study's relevance and importance. Results also show that DRL deployment is more difficult than other DRL issues. Additionally, we built a taxonomy of 31 unique challenges in deploying DRL to different platforms. On all platforms, RL environment-related challenges are the most popular, and communication-related challenges are the most difficult among practitioners. We hope our study inspires future research and helps the community overcome the most common and difficult challenges practitioners face when deploying DRL systems.

==> tables/table_3.tex <==
\begin{table}[htbp]
  \centering
  \caption{Correlation of challenges' popularity and difficulty.}
  \label{tab:correlation}
  \resizebox{0.45\textwidth}{!}{%
  \begin{tabular}{l|c|c}
    \hline
    \textbf{Correlation Coeff. /} & \textbf{Avg. Views} & \textbf{Avg. Scores} \\

    \textbf{p-value} & & \\
     \hline
     \textbf{\% posts with no Accepted} & -0.068/0.716 & -0.266/0.148 \\ 

     \textbf{Answers} & & \\ 

    \textbf{Median Response} & 0.330/0.087& \textbf{0.473/0.011}\\ 

    \textbf{Time (Hours)} & & \\ 
    
    \hline
  \end{tabular}%
  }
\end{table}
